A Survey of Security and Privacy Issues in V2X Communication Systems

Vehicle-to-Everything (V2X) communication is receiving growing attention from industry and academia as multiple pilot projects explore its capabilities and feasibility. With about 50\% of global road vehicle exports coming from the European Union (EU), and within the context of EU legislation around security and data protection, V2X initiatives must consider security and privacy aspects across the system stack, in addition to road safety. Contrary to this principle, our survey of relevant standards, research outputs, and EU pilot projects indicates otherwise; we identify multiple security and privacy related shortcomings and inconsistencies across the standards. We conduct a root cause analysis of the reasons and difficulties associated with these gaps, and categorize the identified security and privacy issues relative to these root causes. As a result, our comprehensive analysis sheds lights on a number of areas that require improvements in the standards, which are not explicitly identified in related work. Our analysis fills gaps left by other related surveys, which are focused on specific technical areas but not necessarily point out underlying root issues in standard specifications. We bring forward recommendations to address these gaps for the overall improvement of security and safety in vehicular communication.

==> s2related_work.tex <==
% !TEX root = v2x_survey_main.tex
% !TeX spellcheck = en-GB

% ========  Section 2 (Option_2)  ==========

\section{Related Work}
\label{sec:related_work}
We first review related work of V2X communication.\footnote{An extended version of this section is available in the online supplemental material, including both relevant survey papers and EU projects.}
In the past years, a number of survey papers on security and privacy
aspects of V2X have been published. 
%Table~\ref{tab:Survey_papers} captures the overview of these surveys. 
The purpose of this section is to highlight the differences of our work compared to them. 
These survey papers can be categorized into three
groups: \raisebox{.5pt}{\textcircled{\raisebox{-.6pt} {1}}} discussion and solutions for generic vehicular network,
\raisebox{.5pt}{\textcircled{\raisebox{-.6pt} {2}}}
surveys that cover both DSRC and C-V2X based solutions, and \raisebox{.5pt}{\textcircled{\raisebox{-.6pt} {3}}} surveys that focus specifically on C-V2X solutions. 

In the first group, Hasan et al.~\cite{hasan2020securing}, van der Heijden et al.~\cite{vanderheijden2018survey}, and Bi{\ss}meyer~\cite{bissmeyer2014thesis} exclusively focus on misbehaviour detection. 
In~\cite{hasan2020securing}, a large part of this survey is dedicated to the discussion on attack and misbehaviour detection mechanisms by classifying and comparing numerous proposals on this subject. 
Survey in~\cite{vanderheijden2018survey} provides in-depth analysis of detection mechanisms, and classify them into two-dimensions. The first dimension is \emph{node-centric vs. data-centric}; the second dimension is \emph{autonomous vs. collaborative}. Based on this classification, misbehaviour detection mechanisms can be categorized into one of the four types. The work in ~\cite{bissmeyer2014thesis} focuses in two main areas: 1) misbehaviour detection, and 2) attacker identification in both local short-term and central long-term scope.

The survey by Badea and Stanciu~\cite{badea2018survey} has a limited focus on security and privacy aspects. The only security related topic is on specific use cases and scenarios such as car sharing. 
Similarly, Ometov and Bezzateev~\cite{ometov2017multi} is not a survey; it is a proposal to apply multi-factor authentication (MFA) in V2X communication. This solution uses reversed Lagrange polynomial from Shamir's secret sharing schema as the building block. 
Wang et al.~\cite{wang2020certificate} focus specifically on the
certificate revocation schemes in V2X communication. They analyse and classify them based on location where the
revocation information has been placed. The entire revocation process is
then divided into three stages: 1) resolution, 2) distribution, and 3) the use of revocation information.

In the second group, Huang et al.~\cite{huang2020recent} treat both security and privacy topics although it is a small part of their paper as the content provides overview of 3GPP specifications on both LTE and 5G-based C-V2X rather than a survey. For security aspect, they discuss basic security services and attack types in vehicular networks, then categorize security solutions from two perspectives: 1) cryptography-based schemes, and 2) trust-based schemes. For privacy solutions, they categorize them into two types: 1) identity privacy preservation, and 2) location privacy preservation.
Alnasser et al.~\cite{alnasser2019cyber} analyse security threats and solutions for both DSRC and LTE-based C-V2X. Their threat analysis includes availability, integrity, confidentiality, authenticity, and non-repudiation aspects. Then, they categorize security solutions including cryptography-based, behaviour/trust-based, and identity-based solutions. 
Ghosal and Conti~\cite{ghosal2020security} provide overview and background of both DSRC/WAVE and 3GPP-based LTE and 5G C-V2X systems, then discuss security challenges by analysing various attack types and how they impact V2X communication. Later, they examine techniques and solutions in specific areas, including symmetric key cryptography, privacy preservation, message authentication.

In the third group, Cao et al.~\cite{cao2019survey} cover overall 5G system security and related topics rather than focusing on 5G-based C-V2X. They describe security and privacy aspects of other vertical applications such as IoT, device-to-device (D2D), and 5G-specific topics such as network slice. Only one section (Sec.VI) is dedicated to security in both LTE and 5G-based C-V2X solutions. In it, security requirements, solutions, and open issues are discussed. 
Muhammad and Safdar~\cite{muhammad2018survey} focus specifically on the authentication mechanism in the context of LTE C-V2X. They enumerate attack types and describe their relevance and corresponding countermeasures. They discuss multiple proposed authentication solutions and analyse how they can meet the needs of C-V2X communication.
Lu et al.~\cite{lu2020v2xreview} focus on security and privacy aspects of LTE and 5G-based C-V2X. Their survey is on challenges in trust, security, and privacy-related issues in C-V2X, followed by discussions on strategies to resolve them. 
The discussion in Lai et al.~\cite{lai2020security} rather narrowly focuses on a specific C-V2X scenario (platooning) rather than more general V2X communication. They propose security solutions, including privacy-preserving platoon group set up, distributed group key management, and cooperative message authentication.
Marojevic~\cite{marojevic2018c} focuses on LTE-based C-V2X, discusses its threat scenarios, lists out associated security requirements, and proposes research directions to satisfy these requirements, along with the needs of further standardization to ensure security mechanisms are in place.
In summary, the examined surveys can be characterized as follows: 
\vspace{-0.1cm}
\begin{itemize}
	\item Analysis of relevant threat scenarios and attack types and their impacts to V2X communication,
	\item Discussion of issues, challenges, and requirements on specific security areas,
	\item Discussion on approaches and strategies to address stated issues and requirements,
	\item Description and comparison of existing proposed solutions on specific security areas,
	\item A new proposal on specific security or privacy area.
\end{itemize}

In contrast to these surveys, as articulated in Sec.~\ref{sec:intro_methodology}, our unique contribution in this paper is to point out fundamental issues and gaps in the ETSI ITS standards and unreported security and privacy issues that have not been discussed in the existing survey papers.
